Fixed Integral Neural Networks

It is often useful to perform integration over learned functions represented by neural networks. However, this integration is usually performed numerically, as analytical integration over learned functions (especially neural networks) is generally viewed as intractable. In this work, we present a method for representing the analytical integral of a learned function $f$. This allows the exact integral of a neural network to be computed, and enables constrained neural networks to be parametrised by applying constraints directly to the integral. Crucially, we also introduce a method to constrain $f$ to be positive, a necessary condition for many applications (e.g. probability distributions, distance metrics, etc). Finally, we introduce several applications where our fixed-integral neural network (FINN) can be utilised.

==> RelatedWork.tex <==
Previous work has shown that integration over learned functions is a powerful tool. It has been used in many disparate applications, from constraining monotonic functions \cite{monotonic} to computing the output of a network over a distribution of parameters \cite{bayesian}. The entire field of Neural ODEs is predicated on the ability to integrate a learned dynamics function over time \cite{neuralode, ffjord, graphode}. However, all of these methods rely on \textit{numerical} integration, which is computationally expensive and not exact.

Another work in the same vein as our method is Hamiltonian Neural Networks \cite{hamiltonian}, which parameterises a vector field which conserves energy by formulating it as the symplectic gradient of an energy function. However, this method is only used as a means of constraining the learned function, not as a technique for integration.
